Factored Policy Gradients: Leveraging Structure for Efficient Learning in MOMDPs

Policy gradient methods can solve complex tasks but often fail when the dimensionality of the action-space or objective multiplicity grow very large. This occurs, in part, because the variance on score-based gradient estimators scales quadratically. In this paper, we address this problem through a factor baseline which exploits independence structure encoded in a novel action-target influence network. Factored policy gradients (FPGs), which follow, provide a common framework for analysing key state-of-the-art algorithms, are shown to generalise traditional policy gradients, and yield a principled way of incorporating prior knowledge of a problem domain's generative processes. We provide an analysis of the proposed estimator and identify the conditions under which variance is reduced. The algorithmic aspects of FPGs are discussed, including optimal policy factorisation, as characterised by minimum biclique coverings, and the implications for the bias-variance trade-off of incorrectly specifying the network. Finally, we demonstrate the performance advantages of our algorithm on large-scale bandit and traffic intersection problems, providing a novel contribution to the latter in the form of a spatial approximation.

==> figures/apples_oranges_diff.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{img/apples_oranges_pdiff.png}

    \caption{Average episodic reward for FPGs and VPGs in the apples and
        oranges environment as a function of $\kappa$ and $\lambda$. Each point
        was computed using the mean over five randomised trials and the 95\%
        confidence interval under a Normal assumption. All differences,
        excluding $(\kappa = 0.1, \lambda = 0.5)$ and $(\kappa = 0.3, \lambda =
        1.0)$, are statistically significant to the 95\% confidence level under
        a two-sample t-test.}\label{fig:apples_oranges:pdiff}
\end{figure*}


==> figures/apples_oranges_learning.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{img/apples_oranges_learning.png}

    \caption{Rolling mean and standard deviation of episodic reward for the
    apples and oranges environment with $\kappa = 0.2$ and $\lambda =
    0.5$.}\label{fig:apples_oranges:learning}
\end{figure}


==> figures/graph_apples_oranges.tex <==
\begin{figure*}[!ht]
    \centering
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \begin{tikzpicture}
            % Define nodes
            \node[obs, minimum size=30pt] (a1) {$\bm{a}^{\textsc{A}}$};
            \node[obs, right=of a1, minimum size=30pt] (a2) {$\bm{a}^{\textsc{O}}$};

            \node (adots) at ($(a1)!0.5!(a2)$) {};
            \node[obs, above=of adots, minimum size=30pt] (penalty) {$P^2$};

            \node[obs, below=of a1, minimum size=30pt] (pnl1) {$Y^\textsc{A}$};
            \node[obs, left=of pnl1, minimum size=30pt] (cost1) {$\dot<\bm{c}^\textsc{A}, \bm{a}^\textsc{A}>$};

            \node[obs, below=of a2, minimum size=30pt] (pnl2) {$Y^\textsc{O}$};
            \node[obs, right=of pnl2, minimum size=30pt] (cost2) {$\dot<\bm{c}^\textsc{O}, \bm{a}^\textsc{O}>$};

            % Connect the nodes
            \edge{a1,a2} {penalty};
            \edge{a1} {pnl1,cost1};
            \edge{a2} {pnl2,cost2};
        \end{tikzpicture}

        \caption{Original influence network.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \begin{tikzpicture}
            % Define nodes
            \node[obs, minimum size=30pt] (a) {$\sigma^\pi\!\left(\bm{a}\right)$};
            \node[obs, above=of a, minimum size=30pt] (penalty) {$P^2$};
            \node[obs, left=of a, minimum size=30pt] (pnl) {$Y$};
            \node[obs, right=of a, minimum size=30pt] (cost) {$\dot<\bm{c}, \bm{a}>$};

            % Connect the nodes
            \edge{a} {penalty,pnl,cost};
        \end{tikzpicture}
        \vspace{4em}

        \caption{Uni-factored influence network.}
    \end{subfigure}
    \\[1.5em]
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \begin{tikzpicture}
            % Define nodes
            \node[obs, minimum size=30pt] (a1) {$\sigma^\pi_\textsc{A}\!\left(\bm{a}\right)$};
            \node[obs, right=of a1, minimum size=30pt] (a2) {$\sigma^\pi_\textsc{O}\!\left(\bm{a}\right)$};

            \node (adots) at ($(a1)!0.5!(a2)$) {};
            \node[obs, above=of adots, minimum size=30pt] (penalty) {$P^2$};

            \node[obs, below=of a1, minimum size=30pt] (pnl1) {$Y^\textsc{A}$};
            \node[obs, left=of pnl1, minimum size=30pt] (cost1) {$\dot<\bm{c}^\textsc{A}, \bm{a}^\textsc{A}>$};

            \node[obs, below=of a2, minimum size=30pt] (pnl2) {$Y^\textsc{O}$};
            \node[obs, right=of pnl2, minimum size=30pt] (cost2) {$\dot<\bm{c}^\textsc{O}, \bm{a}^\textsc{O}>$};

            % Connect the nodes
            \edge{a1,a2} {penalty};
            \edge{a1} {pnl1,cost1};
            \edge{a2} {pnl2,cost2};
        \end{tikzpicture}

        \caption{Bi-factored influence network:
        $\sigma^\pi_\textsc{A}\!\left(\bm{a}\right) \doteq \bm{a}^\textsc{A}$
        and $\sigma^\pi_\textsc{O}\!\left(\bm{a}\right) \doteq
        \bm{a}^\textsc{O}$. Corresponds to a minimum factorisation.}
    \end{subfigure}

    \caption{Influence networks for the apples and oranges problem in terms of
        the rewards components, including the income, cost and (coupled)
        spoilage penalty. Note that the actual algorithm uses targets that are
        defined as the expected discounted sum of future values for each of
    these terms.}\label{fig:graph:apples_oranges}
\end{figure*}

